Identifying Stable Patterns over Time for Emotion Recognition from EEG

In this paper, we investigate stable patterns of electroencephalogram (EEG) over time for emotion recognition using a machine learning approach. Up to now, various findings of activated patterns associated with different emotions have been reported. However, their stability over time has not been fully investigated yet. In this paper, we focus on identifying EEG stability in emotion recognition. To validate the efficiency of the machine learning algorithms used in this study, we systematically evaluate the performance of various popular feature extraction, feature selection, feature smoothing and pattern classification methods with the DEAP dataset and a newly developed dataset for this study. The experimental results indicate that stable patterns exhibit consistency across sessions; the lateral temporal areas activate more for positive emotion than negative one in beta and gamma bands; the neural patterns of neutral emotion have higher alpha responses at parietal and occipital sites; and for negative emotion, the neural patterns have significant higher delta responses at parietal and occipital sites and higher gamma responses at prefrontal sites. The performance of our emotion recognition system shows that the neural patterns are relatively stable within and between sessions.

==> README <==
January 10, 2007

Please note that you may choose to use either double column or single column
formatting. You may wish to use single column formatting when submitting your
paper for review, as it leaves more space for reviewer remarks. The double column format 
is ideal when submitting your final publication materials. The IEEE CS formats articles
in two columns, with 9.5pt Palatino font, and a page size of 7.875 X 10.75. 

June 6, 2006

Added an option to switch between peer review and final submission formats 
into bare_jrnl.tex. 


August 13, 2002

This IEEEtran.cls is the official LaTeX class for authors of the
Institute of Electrical and Electronics Engineers (IEEE) transactions
journals and conferences. In addition to being carried on IEEE's site,
IEEEtran.cls may be found at:

http://www.ctan.org/tex-archive/macros/latex/contrib/supported/IEEEtran/

The CTAN site may have additional files related to non-IEEE uses of this
tool.

As of version 1.6, IEEEtran.cls now provides support for conferences and
A4 paper. Users of previous versions should no longer manually alter margins,
paper sizes, page styles, etc. Also, please note that \author is used
slightly differently from that of V1.5, especially for conferences.
\pubid (if used) must now be placed before \maketitle. \cite is now robust
and can be used within captions without a proceeding \protect.

As with previous versions, The itemize, enumerate, and description lists as
well as \appendix(ces) have enhanced controls and work slightly differently
than is done in traditional LaTeX.

Extensive formal documentation is now available. Enjoy! ;) The appendices
of the user manual contain important information on avoiding commonly
made mistakes, compatibility issues and installation instructions.


Best wishes for all your publication endeavors,

Michael Shell
mshell@ece.gatech.edu



********************* Files **********************

README               - This file.

IEEEtran.cls         - The LaTeX class file.

IEEEtran_HOWTO.pdf   - The user manual.

bare_jrnl.tex        - A "bare bones" starter file for journal papers.




**********************************************************************
 Legal Notice:
 This code and advice is offered as-is without any warranty either
 expressed or implied; without even the implied warranty of
 MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE!
 User assumes all risk.
 In no event shall IEEE or any contributor to this code
 be liable for any damages or losses, including, but not limited to,
 incidental, consequential, or any other damages, resulting from the
 use or misuse of any information contained here.
 
 All statements made here are the opinions of their respective
 authors and are not necessarily endorsed by the IEEE.

 This code/text is distributed under the Perl Artistic License 
 ( http://language.perl.com/misc/Artistic.html ) 
 and may be freely used, distributed and modified.
 Retain all contribution notices and credits.
**********************************************************************



